Distributed Multi-Relay Selection in Accumulate-then-Forward Energy Harvesting Relay Networks

This paper investigates a wireless-powered cooperative network (WPCN) consisting of one source-destination pair and multiple decode-and-forward (DF) relays. We develop an energy threshold based multi-relay selection (ETMRS) scheme for the considered WPCN. The proposed ETMRS scheme can be implemented in a fully distributed manner as the relays only need local information to switch between energy harvesting and information forwarding modes. By modeling the charging/discharging behaviours of the finite-capacity battery at each relay as a finite-state Markov Chain (MC), we derive an analytical expression for the system outage probability of the proposed ETMRS scheme over mixed Nakagami-$m$ and Rayleigh fading channels. Based on the derived expression, the optimal energy thresholds for all the relays corresponding to the minimum system outage probability can be obtained via an exhaustive search. However, this approach becomes computationally prohibitive when the number of relays and the associated number of battery energy levels is large. To resolve this issue, we propose a heuristic approach to optimize the energy threshold for each relay. To gain some useful insights for practical relay design, we also derive the upper bound for system outage probability corresponding to the case that all relays are equipped with infinite-capacity batteries. Numerical results validate our theoretical analysis. It is shown that the proposed heuristic approach can achieve a near-optimal system performance and our ETMRS scheme outperforms the existing single-relay selection scheme and common energy threshold scheme.

==> performance_analysis.tex <==
\section{System Performance Analysis and Optimization}
Based on the stationery discrete distribution of relay batteries derived in Sec. III, in this section we first analyze the system outage probability of the proposed ETMRS scheme. Based on the derived closed-form expression, we subsequently discuss how to optimize the energy threshold of the relays to minimize the system outage probability.

\subsection{Outage Probability Analysis}
Let ${\rm O}$ denote the outage event of the considered system employing the proposed ETMRS scheme. According to the full probability theory, we can express the system outage probability~as %\cite{selection}
\begin{equation}\label{outage}
P_{\rm{out}} = \Pr \left\{ \rm O \right\} = \sum\limits_{\Phi  \in \Lambda } {\Pr \left\{ \Phi  \right\}} \Pr \left\{ {{\rm O}\left| \Phi  \right.} \right\},
\end{equation}
where $\Lambda  = \left\{ {R_1 ,R_2  \cdots ,R_N } \right\}$ denotes the set of all relays in the considered network and incorporates the decoding set $\Phi$ as its subset, $\Pr \left\{ \Phi  \right\}$ denotes the probability that the current decoding set is $\Phi$, and $\Pr \left\{ {{\rm O}\left| \Phi  \right.} \right\}$ denotes the probability that system outage occurs under the decoding set $\Phi$. In order to further expand (\ref{outage}), we define ${\Phi _{k,n}}$ to denote the $n$-th $k$-subset of $\Lambda$ (i.e., the $n$-th $k$-subset of $\Lambda$ contains exactly $k$ elements, $k = 1, 2, \cdots ,N$, $n = 1,2, \cdots ,\binom{N}{k}$). Then the outage probability of the ETMRS scheme can be further expanded as
\begin{equation}\label{outage1}
P_{\rm{out}} = \Pr \left\{ \emptyset \right\} + \sum\limits_{k = 1}^N {\sum\limits_{n = 1}^{\binom{N}{k}} {\Pr \left\{ {{\Phi _{k,n}}} \right\}\Pr \left\{ {{\rm O}\left| {{\Phi _{k,n}}} \right.} \right\}}},
\end{equation}
by realizing that the system outage probability equals to one when the decoding set is an empty set $\emptyset$. The empty decoding set can be caused by two kinds of event: One is that none of the relays working in IF mode decodes the received signal from source correctly. The other is that  all relays operate in EH mode and no relay performs IF. Based on the derived stationary discrete distribution of relay batteries given in (\ref{app-energy-distri}), we can calculate the first probability term in (\ref{outage1}) as follows
\begin{equation}\label{firstterm}
\begin{split}
\Pr \left\{ \emptyset   \right\}  &= \prod\limits_{u:R_u  \in \Lambda } {\Pr \bigg\{ {\left\{ {\zeta _u  = \zeta _I ,\varphi _u  = 0} \right\} \cup \zeta _u  = \zeta _E } \bigg\}}   \\
   &= \prod\limits_{u:R_u  \in \Lambda } { \left( {\Pr \left\{{\varphi_u = 0}\right\} \sum\limits_{i =  {\chi_u}/\varepsilon_1}^L {\pi _{u,i} }  + \sum\limits_{i = 0}^{ {\chi_u}/\varepsilon_1 }{\pi _{u,i} }}\right)}.  \\
\end{split}
\end{equation}
Similarly, the term $\Pr\left\{{\Phi_{k,n}}\right\}$ can be computed as
\begin{equation}\label{secondterm}
\begin{split}
& \quad \Pr \left\{ {{\Phi _{k,n}}} \right\} \\
&= \prod\limits_{u:R_u  \in \Phi_{k,n} } {\Pr \left\{ {\zeta _u  = \zeta _I ,\varphi _u  = 1} \right\}}  \prod\limits_{u:R_u  \notin \Phi_{k,n} } {\Pr \bigg\{ {\left\{ {\zeta _u  = \zeta _I ,\varphi _u  = 0} \right\} \cup \zeta _u  = \zeta _E } \bigg\}}   \\
  &  = \prod\limits_{u:R_u  \in \Phi_{k,n} } { \left[{\left( {1 - \Pr \left\{{\varphi_u = 0}\right\}} \right)\sum\limits_{i ={\chi_u}/\varepsilon_1 }^L {\pi _{u,i} } } \right]}\  \prod\limits_{u:R_u  \notin \Phi_{k,n}} { \left( {\Pr \left\{{\varphi_u = 0}\right\} \sum\limits_{i = { {\chi_u}}/\varepsilon_1}^L {\pi _{u,i} }  + \sum\limits_{i = 0}^{ {\chi_u}/\varepsilon_1 }{\pi _{u,i} }}\right)} .  \\
\end{split}
\end{equation}

To evaluate the third probability term in (\ref{outage1}), we first characterize the distribution of the conditional end-to-end SNR for a given decoding set. For notation simplicity, we use $\gamma_{k,n}$ to denote the received SNR at the destination when the decoding set is $\Phi_{n,k}$. Recall that the conditional end-to-end SNR for a certain decoding set is given in (\ref{snr}), which includes a weighted sum of Rayleigh random variables. However, to the best knowledge of authors, the exact distribution of a weighted sum of Rayleigh random variables does not exist in open literature. As a result, we cannot further characterize the exact distribution of $\gamma_{k,n}$. Fortunately, with the aid of a tight approximation for the CDF of a weighted sum of Rayleigh random variables derived in \cite{appro2}, the CDF of $\gamma_{k,n}$ can be approximated as a gamma distribution and expressed as
\begin{equation}\label{5}
{F_{\gamma_{k,n}}} \left({x}\right) \approx  {{\gamma \left( {k,{{{{{{N_0}} \over { 4\sum\limits_{u:{R_u} \in {\Phi _{k,n}}} {{\beta _u}{\sigma _u^2}} } }}} }x} \right)} \over {\Gamma \left( k \right)}},
\end{equation}
where $\sigma_u = \sqrt {{\lambda _{{R_u}D}}/2}$ is the scale parameter of the Rayleigh fading channel between $R_u$ and~$D$.

\begin{table}
\centering \scalebox{0.40}{\includegraphics{table.eps}}
\caption{The relation between $\phi _{k,n,j}$ and $\sqrt{{\beta_u} }\sigma_u$, $u = 1,2, \cdots ,N$, for $k = 1, \cdots ,N$, $n = 1,2, \cdots ,\binom{N}{k} $ and $j = 1,2, \cdots ,k$. }\label{table:1}
\end{table}
In order to further expand the summation term in (\ref{5}), we use a similar method adopted in \cite{tablewtf,cl_chen,PRS}. To this end, we define a set ${\rm A}=\bigg\{ { \sqrt{ {\beta_u}}{\sigma_u}:{R_u} \in \Lambda ,u \in \left\{ {1,2, \cdots ,N} \right\}} \bigg\}$ with the same cardinality as the set $\Lambda$ (i.e., $\left| \rm A  \right| = \left| \Lambda  \right|$ ). Similarly, let ${\rm A}_{k,n}$ denote the $n$-th $k$-subset of $\rm A$. The $j$-th element of the subset ${\rm A}_{k,n}$ are denoted by $\phi _{k,n,j} \in {\rm A}_{k,n}$, $j = 1,2, \cdots ,k$. To be more clear, we list the corresponding relationship between $\phi _{k,n,j}$ and $\sqrt{{\beta_u} }\sigma_u$ in Table I.

With the corresponding relation between $\phi _{k,n,j}$ and $\sqrt{ {\beta_u} }\sigma_u$, (\ref{5}) can now be expressed as
\begin{equation}\label{condcdfsnr}
{F_{\gamma_{k,n}}} \left({x}\right) \approx  {{\gamma \left( {k,{a_{k,n}}x} \right)} \over {\Gamma \left( k \right)}}= 1 - \exp ( - a_{k,n} x) \sum\limits_{i = 0}^{k - 1} {{\left({a_{k,n} x}\right)^{i} } \over {i!}},
\end{equation}
where $a_{k,n}= {{{{{{N_0}} \over { 4 \sum\limits_{j = 1}^k {\phi_{k,n,j}^2}} }}} }$ and the last equality in (\ref{condcdfsnr}) holds according to \cite[Eq. (8.352.6)]{Tableofintegral} with integer $k$.
Based on the distribution of $\gamma_{k,n}$, the third probability term in (\ref{outage1}) can now be further expanded~as
\begin{equation}\label{2}
\begin{split}
& \Pr \left\{ {{\rm O}\left| \Phi_{k,n}  \right.} \right\} =  \Pr\left\{  {\gamma_{k,n}}< {v }\right\} ={F_{\gamma_{k,n}}}\left({v}\right) \approx 1 - \exp ( - a_{k,n} v) \sum\limits_{i = 0}^{k - 1} {{\left({a_{k,n} v}\right)^{i} } \over {i!}}.
\end{split}
\end{equation}
By substituting (\ref{firstterm}), (\ref{secondterm}) and (\ref{2}) into (\ref{outage1}), we have derived an approximate closed-form expression of the outage probability for the proposed ETMRS scheme.



In terms of the i.i.d channel fading case where the relays have the same energy threshold, the number of different decoding sets reduces to $N+1$ and the expression of system outage probability can be simplified to
\begin{equation}\label{iid1}
\mathord{\buildrel{\lower3pt\hbox{$\scriptscriptstyle\frown$}}\over
 P  }_{\rm{out}}= \Pr \left\{ \rm O \right\} = \Pr \left\{{ {\mathord{\buildrel{\lower3pt\hbox{$\scriptscriptstyle\frown$}}\over
 \emptyset  } }}\right\}  + \sum\limits_{k = 1}^N { {\Pr \left\{{ {{\mathord{\buildrel{\lower3pt\hbox{$\scriptscriptstyle\frown$}}\over\Phi} _{k}}} }\right\}\Pr \left\{{ {{\rm O}\left| {{\mathord{\buildrel{\lower3pt\hbox{$\scriptscriptstyle\frown$}}\over\Phi} _{k}}} \right.} }\right\}}},
\end{equation}
where $\Pr \left\{ {\mathord{\buildrel{\lower3pt\hbox{$\scriptscriptstyle\frown$}}\over
 \emptyset  } }\right\}$ is the probability that the decoding set is empty for the i.i.d. case, $\Pr \left\{ {{\mathord{\buildrel{\lower3pt\hbox{$\scriptscriptstyle\frown$}}\over\Phi} _{k}}} \right\}$ is the probability that the decoding set contains $k$ relays, and ${\Pr \left\{ {{\rm O}\left| {{\mathord{\buildrel{\lower3pt\hbox{$\scriptscriptstyle\frown$}}\over\Phi} _{k}}} \right.} \right\}}$ is the conditional outage probability when $k$ relays falls in the decoding set. Similar to the analysis of the general case, the first and second probability terms in (\ref{iid1}) can be expressed as
\begin{equation}\label{firsttermiid}
\begin{split}
\Pr \left\{ {\mathord{\buildrel{\lower3pt\hbox{$\scriptscriptstyle\frown$}}\over
 \emptyset  } }\right\} =  \left( {\Pr \left\{{\varphi = 0}\right\} \sum\limits_{i =  {\chi}/\varepsilon_1}^L {\pi _{i} }  + \sum\limits_{i = 0}^{ {\chi}/\varepsilon_1 }{\pi _{i} }}\right)^N, \\
\end{split}
\end{equation}
\begin{equation}\label{secondtermiid}
\begin{split}
\Pr \left\{ {{\mathord{\buildrel{\lower3pt\hbox{$\scriptscriptstyle\frown$}}\over\Phi }_{k}}} \right\} =   {\binom{N}{k}} \left[{\left( {1 - \Pr \left\{{\varphi = 0}\right\} } \right)\sum\limits_{i ={\chi}/\varepsilon_1 }^L {\pi _{i} } } \right]^k  \left( {\Pr \left\{{\varphi = 0}\right\} \sum\limits_{i = { {\chi}}/\varepsilon_1}^L {\pi _{i} }  + \sum\limits_{i = 0}^{ {\chi}/\varepsilon_1 }{\pi _{i} }}\right)^{N-k}, \\
\end{split}
\end{equation}
where $\chi = \alpha+\beta$ is the identical energy threshold for all the relays and $\Pr \left\{{\varphi = 0}\right\}$ is the outage probability of the relays for the special i.i.d. channel fading case, which can be derived from that for the general case given in (\ref{general}) and written as
\begin{equation}
\Pr \left\{{\varphi = 0}\right\} = {{\gamma \left( {m,  {m v N_0 \over {\lambda_{SR} P}}} \right)} \over {\Gamma \left( m \right)}},
\end{equation}
where $m$ is the identical severity parameter of the Nakagami-m fading channels between source and relays and ${\lambda_{SR}}$ is the identical channel power gain of the first hop.

The third probability term in (\ref{iid1}) can be deduced from (\ref{2}) as
\begin{equation}\label{snriid}
\Pr \left\{{ {{\rm O}\left| {{\mathord{\buildrel{\lower3pt\hbox{$\scriptscriptstyle\frown$}}\over\Phi} _{k}}} \right.} }\right\} \approx 1 - \exp ( - {{{{{{N_0v}} \over { 4 k \beta \sigma^2} }}} }) \sum\limits_{i = 0}^{k - 1} {{\left({{{{{{{N_0v}} \over { 4 k \beta \sigma^2} }}} }}\right)^{i} } \over {i!}},
\end{equation}
where $\sigma= \sqrt {\lambda_{RD} /2} $ is the identical scale parameter for the Rayleigh fading channels between relays and destination. Note that different from (\ref{2}), the expression of the conditional system outage probability given in (\ref{snriid}) does not require the parameters defined in Table I. The outage probability for the special i.i.d. channel fading case can be obtained by substituting (\ref{firsttermiid}), (\ref{secondtermiid}) and (\ref{snriid}) into (\ref{iid1}).

{\color{blue}
\subsection{Energy Threshold Optimization}
We first consider the special i.i.d. channel fading case where the associated energy thresholds for all the relays is identical, denoted by $\chi = \alpha+\beta$. When $\beta$ grows, the conditional outage probability derived in (\ref{snriid}) reduces and the overall system outage probability correspondingly decreases. On the other hand, according to (\ref{secondtermiid}), increasing the energy threshold $\beta$ will lead to an increase of $\chi$ and thus decrease the probability of each relay working in IF mode and the number of relays falling into the decoding set. This will increase the overall system outage probability. In simple words, when the designed energy threshold $\chi$ for the relays is small, most of relays could fall into the decoding set but their transmit power is low. When the energy threshold is large, only a few relays fall into the decoding set but their associated transmit power is high. We can now infer that for the special i.i.d. channel fading case, there must exist an optimal energy threshold $\chi \in \left\{\varepsilon _{1}, \varepsilon _{2},\cdots, \varepsilon _{L} \right\}$ that minimize the system outage probability of the proposed ETMRS scheme. Similarly, for the general i.n.i.d. channel fading case where the relays may be located quite differently. There should also exist an optimal energy threshold set $\left\{\chi_1, \chi_2,\cdots,\chi_N\right\}, \chi_u \in \left\{\varepsilon _{1}, \varepsilon _{2},\cdots, \varepsilon _{L} \right\}, \forall u=1,2,\cdots,N$, for all relays that minimize the overall system outage probability.

Due to the complexity of the adopted MC model, it is difficult to derive a closed-form expression for the optimal energy threshold of each relay. However, for the special i.i.d. channel fading case, the optimal energy threshold can be easily achieved by performing a one-dimension exhaustive search from all the possible energy levels with the derived analytical outage probability given in (\ref{iid1}). The computation complexity of this search is given by $O\left(L\right)$.

When it comes to the general i.n.i.d. case, the optimal set of energy thresholds can be found by a $N$-dimension exhaustive search from all the possible combinations of energy thresholds with the analytical expression derived in (\ref{outage1}). The computation complexity is $O\left(L^N\right)$, which grows exponentially with the number of relays $N$. Thus, finding the optimal set of energy thresholds becomes computationally prohibitive when the number of relays $N$ and the level of batteries $L$ are large. To overcome this problem, in the following subsection, we provide a heuristic approach to design the energy thresholds for the general i.n.i.d. case.


\subsection{A Heuristic Approach for i.n.i.d Scenario}
Intuitively, a higher energy threshold should be set for those relays closer to the source node. This is because that the average amount of harvested energy is higher for those relays and they can support a higher transmit power to reduce the overall system outage probability. On the other hand, relays closer to the source node are relatively farer away from the destination node such that the associated second hop channels are relatively weaker, a higher energy threshold should also be used to overcome the larger path loss. Similarly, for the relays near the destination node, smaller energy thresholds can be adopted due to their limited harvested energy and stronger second hop channels. Inspired by this fact, we design the energy threshold for each relay $R_u$ in the considered network as
\begin{equation}
\tilde \chi_u = z \lambda_{S{R_u}} / \lambda_{{R_u}D},
\end{equation}
where $z$ is a scalar factor to adjust the overall transmit power of all the relays. For the considered discrete-battery model, the designed energy threshold $\tilde \beta_u$ must be discretized to one specific energy level of the battery. We define the discretized energy threshold for the $u$-th relay~as
\begin{equation}\label{dif}
{\chi_u} \buildrel \Delta \over = {\varepsilon _{j}}, \quad \text{where} \quad j=
\left\{
\begin{matrix}
\begin{split}
&\arg \mathop {\min }\limits_{i \in \left\{ {0,1, \cdots ,L} \right\}} \bigg\{{\varepsilon _i}:{\varepsilon _i} \ge \tilde {\chi_u}\bigg\}, \quad \text{if} \quad \tilde {\chi_u} \le {\varepsilon _L} \\
&L,  \quad \text{if} \quad \tilde {\chi_u} > {\varepsilon _L}
\end{split}
\end{matrix}
\right..
\end{equation}
Based on the above definitions, the discretized energy threshold for relay $R_u$ can be further expressed as
\begin{equation}\label{threshold}
{\chi_u}=  \min \left( {{\varepsilon _1}\left\lceil {z  \lambda_{S{R_u}} \over {\lambda_{R_u D} {\varepsilon _1}}} \right\rceil ,C} \right).
\end{equation}


Similar to the analysis given in the previous subsection, we can deduce that there should exist an optimal value of $z$ that minimize the system outage probability. To find the optimal value of $z$,  we first define $\lambda_{\max} $ and $\lambda_{\min}$ as the maximum and minimum value of the term $\lambda_{S{R_u}} / \lambda_{{R_u}D}$, among all relays, respectively. The optimal $z$ should exist within the interval $\left[{{\varepsilon _1}/\lambda_{\max}  , {{\varepsilon _L}/\lambda_{\min} } }\right]$, where $z = {\varepsilon _1}/\lambda_{\max}$ could make all relays choose $\varepsilon_1$ as their energy thresholds and $ z = {{\varepsilon _L}/\lambda_{\min} }$ will force all relays to adopt energy level $L$ as their energy thresholds. The optimal $z$ thus can now be achieved by performing a one-dimension exhaustive search from this interval over the derived outage probability expression. In order to capture all the possible combinations, we search $z$ with an increment of ${\varepsilon _1}/\lambda_{\max}$ each time and the computation complexity for the proposed heuristic approach can be expressed by $O\left(L\lambda_{\max}/\lambda_{\min}\right)$. Note that the complexity of the heuristic approach is obviously much lower than that of the exhaustive search given by $O\left(L^N\right)$.
}



